Exploring Multi-Grained Concept Annotations for Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) excel in vision--language tasks by pre-training solely on coarse-grained concept annotations (e.g., image captions). We hypothesize that integrating fine-grained concept annotations (e.g., object labels and object regions) will further improve performance, as both data granularities complement each other in terms of breadth and depth in concept representation. We introduce a new dataset featuring Multimodal Multi-Grained Concept annotations (MMGiC) for MLLMs. In constructing MMGiC, we explore the impact of different data recipes on multimodal comprehension and generation. Our analyses reveal that multi-grained concept annotations integrate and complement each other, under our structured template and a general MLLM framework. We clearly explore and demonstrate the potential of MMGiC to help MLLMs better locate and learn concepts, aligning vision and language at multiple granularities. We further validate our hypothesis by investigating the fair comparison and effective collaboration between MMGiC and image--caption data on 12 multimodal comprehension and generation benchmarks, e.g., their appropriate combination achieve 3.95% and 2.34% absolute improvements over image--caption data alone on POPE and SEED-Bench. Code, data and models will be available at https://github.com/LooperXX/MMGiC.

==> tables/oi-oi-ic-init.tex <==
\begin{table}[t]
    \centering
    \tablestyle{6pt}{1.2}
    \caption{
        Zero-shot evaluation of different data recipes of the first training phase.
        For each group, the best result are \textbf{bold}.
        CLIP-T/I: image--text or image-image similarity via CLIP; $\downarrow$: lower is better, otherwise higher is better.
    }
    \label{tab:oi_oi_ic_init}
    \scalebox{0.9}{
        \begin{tabular}{c|l|cc|rcccc}
            \toprule
            & \multirow{3}{*}{{Training Data}} & \multicolumn{2}{c|}{{Image  Captioning}} & \multicolumn{5}{c}{{Image Generation}} \\
            & {} & COCO & NoCaps & \multicolumn{3}{c}{MS-COCO-30K} & \multicolumn{2}{c}{VIST} \\
            \cmidrule{3-9}
            & {} & CIDEr & CIDEr & FID ($\downarrow$) & CLIP-T & CLIP-I & FID ($\downarrow$)& CLIP-I \\
            \midrule
            \textcolor{indexcolor}{0} & \datasetname{} $\rightarrow$ \icdatasetname{} & \textbf{105.62} & { }{ }\textbf{93.77} & \textbf{7.29} & \textbf{31.57} & \textbf{70.26} & \textbf{37.45} & \textbf{65.88} \\

            \textcolor{indexcolor}{1} & \datasetnamecaptiononly{} $\rightarrow$ \icdatasetname{} & 105.33 & { }{ }92.93 & 7.54 & 31.45 & 70.00 & 41.76 & 65.17 \\


            \hdashline

            \textcolor{indexcolor}{2} & {\datasetname{}$+$\icdatasetname{} $\rightarrow$ \datasetname{}} & \textbf{121.22} & 105.33 & \textbf{7.22} & 31.91 & \textbf{71.75} & \textbf{36.23} & \textbf{65.79} \\
        
            \textcolor{indexcolor}{3} & {\datasetnamecaptiononly{}$+$\icdatasetname{} $\rightarrow$ \datasetname{}} & 120.61 & \textbf{105.42} & 7.30 & \textbf{31.95} & 71.46 & 37.08 & 65.65 \\
            
            \bottomrule
        \end{tabular}
    }
\end{table}

==> tables/sft_generation.tex <==
\begin{table}[t]
    \centering
    \tablestyle{4pt}{1.1}
    \caption{
        Zero-shot evaluation of different baselines on multimodal generation benchmarks after SFT.
        MLLMs in Group \textcolor{indexcolor}{a} are instruction-tuned for multimodal generation only, while MLLMs in Group \textcolor{indexcolor}{b} can be used for both multimodal comprehension and generation.
        DINO: cosine similarity between generated and real images via DINO~\citep{caron2021emerging}; $^{*}$: not tuned on instruction data.
    }
    \label{tab:sft_generation}
    \scalebox{0.85}{
        \begin{tabular}{c|l|ccc|cc|ccc}
            \toprule
            & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{MS-COCO-30K} & \multicolumn{2}{c|}{VIST} & \multicolumn{3}{c}{DreamBench} \\
            &  & {FID} ($\downarrow$) & CLIP-T & CLIP-I & {FID} ($\downarrow$) & CLIP-I & CLIP-T & CLIP-I & DINO \\
            \midrule
            \multicolumn{10}{l}{\demph{\it{SOTA MLLMs, Not Comparable with Our Baselines}}}\\
            \midrule
            \multirow{3}{*}{\textcolor{indexcolor}{a}} & \demph{\textsc{Kosmos-G}}~\citep{pan2023kosmosg} & \demph{10.99} &  &  &  &  & \demph{28.70} & \demph{84.70} & \demph{69.40} \\
            & \demph{GILL}~\citep{koh2024generating} & \demph{12.20} &  &  &  & \demph{64.10} &  &  &  \\
            & \demph{Emu2-Gen-37B}~\citep{sun2023generative2} &  & \demph{29.70} & \demph{68.60} &  &  & \demph{28.70} & \demph{85.00} & \demph{76.60} \\
            \hdashline
            \multirow{3}{*}{\textcolor{indexcolor}{b}} & \demph{VL-GPT-I-7B}~\citep{zhu2023vl} & \demph{11.53} &  &  &  &  &  &  &  \\
            & \demph{LaVIT-v2-7B$^{*}$}~\citep{jin2023unified} & \demph{{ }{ }7.10} & \demph{31.93} & \demph{71.06} & \demph{34.76} & \demph{68.41} &  &  &  \\
            & \demph{SEED-LLaMA-I-8B}~\citep{ge2023making} & \demph{16.66} & \demph{29.52} & \demph{69.22} & \demph{43.69} & \demph{65.21} & \demph{27.06} & \demph{79.27} & \demph{54.42} \\
            \midrule
            \multicolumn{10}{l}{\it{Our Comparable Baselines}}\\
            \midrule
            \textcolor{indexcolor}{0} & \methodnameic{} & { }{ }8.11 & 30.90 & 70.72 & 38.19 & 65.37 & 27.50 & \underline{82.92} & \underline{67.41} \\
            \textcolor{indexcolor}{1} & \methodname{} & { }{ }\textbf{6.79} & \textbf{31.63} & \textbf{72.44} & \textbf{34.32} & \textbf{67.66} & \textbf{27.69} & 82.62 & 67.36 \\
            \textcolor{indexcolor}{2} & \methodnamewithic{} & { }{ }\underline{7.29} & \underline{31.54} & \underline{72.03} & \underline{34.39} & \underline{67.19} & \underline{27.62} & \textbf{83.06} & \textbf{68.30} \\
            \bottomrule
        \end{tabular}
    }
\end{table}

